Search-based Motion Planning for Quadrotors using Linear Quadratic Minimum Time Control

In this work, we propose a search-based planning method to compute dynamically feasible trajectories for a quadrotor flying in an obstacle-cluttered environment. Our approach searches for smooth, minimum-time trajectories by exploring the map using a set of short-duration motion primitives. The primitives are generated by solving an optimal control problem and induce a finite lattice discretization on the state space which can be explored using a graph-search algorithm. The proposed approach is able to generate resolution-complete (i.e., optimal in the discretized space), safe, dynamically feasibility trajectories efficiently by exploiting the explicit solution of a Linear Quadratic Minimum Time problem. It does not assume a hovering initial condition and, hence, is suitable for fast online re-planning while the robot is moving. Quadrotor navigation with online re-planning is demonstrated using the proposed approach in simulation and physical experiments and comparisons with trajectory generation based on state-of-art quadratic programming are presented.

==> tex/old/DeterministicShortestPath.tex <==
\section{Discretized Motion Primitives}
\label{sec:dsp}
Let $\mathcal{U}_M:=\{u_1,\ldots,u_M\} \subset \mathcal{U}$ be a lattice discretization of the control space $\mathcal{U}$ so that $u_m \in \mathbb{R}^3$. Given an initial state $x_0 := x(0)$, we generate motion primitives of duration $\tau > 0$ that apply a constant control input $u(t) \equiv u_m \in \mathcal{U}_M$ by integrating
\begin{equation}\label{eq: dd}
p^{(n)}_D(t) = u_m
\end{equation}
with the boundary value $x_0$. We use notation
\begin{equation}
x(t) = f(x_0, u)
\end{equation}
to stand for the trajectory derived from the initial state $x_0$ and a known control input sequence $u$.
 We provide explicit expressions for the first-order \emph{(Kinematic)} and second-order \emph{(Dynamic)} models that we use in the paper:

\subsubsection{Kinematic Model}
Assume the state space is $x = [p^\T, v^\T]^\T \in \mathbb{R}^6$ , our control input is the acceleration as $u = a$.  We are able to sample the acceleration as a finite number of $M$ control inputs $u_m = a_m, m = 1,\ldots,M$ which are constant during that primitive.

Let $x_0 = [p_0^\T, v_0^\T]^\T$ be the initial state, integrating Eq.~\eqref{eq: dd} with the boundary value $x_0$ and control input $a_m$ derives
\begin{equation}\label{eq: kk}
x(t) = f(x_0, a_m) = \left[ {\begin{array}{c}
\frac{a_m}{2}t^2+v_0t+p_0\\
a_mt+v_0
\end{array}}\right]
\end{equation}

This result is equivalent to Eq.~\eqref{eq: acc_s}, where $d_3$ is deprecated to zero and the control input is a constant as $u^*(t) = d_2 = a_m$.

\subsubsection{Dynamic Model}
Assume the state space is $x = [p^\T, v^\T, a^\T]^\T \in \mathbb{R}^9$ , our control input is corresponding to the jerk as $u = j$. We are able to sample the jerk as a finite number of $M$ control inputs $u_m = j_m, m = 1,\ldots,M$ which are constant during that primitive.

Similarly, define the boundary value $x_0 = [p_0^\T, v_0^\T, a_0^\T]^\T$, and apply the control input $j_m$ to yield the trajectory by integrating Eq.~\eqref{eq: dd} as
\begin{equation}
x(t) = f(x_0, j_m) = \left[ {\begin{array}{c}
\frac{j_m}{6}t^3+\frac{a_0}{2}t^2+v_0t+p_0\\
\frac{j_m}{2}t^2+a_0t+v_0\\
j_mt+a_0
\end{array}}\right]
\end{equation}

This result is equivalent to Eq.~\eqref{eq: jrk_s}, where $d_5, d_4$ are deprecated to zero and the control input is a constant as $u^*(t) = d_3 = j_m$.


In a nut shell, our motion primitive based on discretized control input is also the optimal trajectory that connect the initial state to the corresponding end state.

\subsection{State Discretization}\label{sec:dis}
Since our control input is discretized, the end states of motion primitives from a given initial state $x_0$ is also discretized given constant trajectory time $\tau$. When we treat the dynamic constraints on velocity, acceleration, etc on each axis independently, the discretization can be calculated with respect to $\tau$ and the discretization step $d_u$ in control space. For example, let $u_{max}$ be the maximum control input in each axis ($\|u\|_\infty \leq u_{max}$), we can set $d_u = \frac{u_{max}}{m_{max}}$ where $m_{max}$ indicates how many samples the user want to achieve from $0$ to $u_{max}$ in each axis. And the total number of sampled primitives are $M = (2m_{max}+1)^n$ (from $-u_{max} to u_{max}$). An example is given in Fig.~\ref{fig: prs} in which we use 9 uniformed samples for 2-D primitives. The way we set the control input constraints will result in a region for possible end states (encompassed by the red bracket in Fig.~\ref{fig: prs}).
\begin{figure}[htp]
  \centering
  \subfigure[Discretized Acceleration.]{\includegraphics[width=0.45\columnwidth, trim=0 0 0 0, clip=true]{./fig/vel.pdf}\label{fig: vel}}
  \subfigure[Discretized Jerk.]{\includegraphics[width=0.45\columnwidth, trim=0 0 0 0, clip=true]{./fig/acc.pdf}\label{fig: acc}}
   \caption{Example of 9 motion primitives from initial state $x_0$ for \textit{Kinematic} (left) and \textit{Dynamic} models (right). The black arrow indicate the control inputs for individual primitive. Red bracket shows the feasible region of end states regarding the maximum control inputs. The initial state has velocity $v_0 = [1, 0, 0]^\T$ and acceleration $a_0 = [0, 1, 0]$ (only for the right figure). \label{fig: prs}}
\end{figure}

Once $d_u$ is designed, we are able to calculate the minimum gap between state space by integrating $d_u$ with respect to time $\tau$. For example, for \textit{Kinematic} model, the resolution for velocity $d_v$ and position $d_p$ can be defined as
\begin{align*}
d_v = d_u\tau \\
d_s = \frac{d_u}{2}\tau^2
\end{align*}

\subsection{Primitive Cost}
The cost of each optimal primitive $x^*(t)$ is analytically defined given the time $\tau$ and control input in Eq.~\eqref{eq: problem0} as
\begin{align}\label{eq: C}
C(x(t),u(t)) =\;& ({\|u_m\|^2} + \rho )\tau
\end{align}
Here we use $u_m$ to emphasize that the control input is a constant in the discrete control space $\mathcal{U}_M$. Obviously, the primitive cost is not a function of $t$, and since we have discretized $u_m$, the cost of each primitive is also discretized.


%Need to describe:
%\begin{itemize}
%  \item Collision checking: piecewise-linear polynomial approximation
%  \item Heuristic:
%  \item Scaling from $U \subset [-1,1]^3$ to $U \subset \mathcal{X}_{(3n-2):3n}$
%\end{itemize}


==> tex/old/HeuristicNikolay.tex <==
\section{Nikolay's Heuristic}
To derive a consistent heuristic for the deterministic shortest path problem in \eqref{eq: problem3}, we consider a relaxation of the original problem in Eq.~\eqref{eq: problem1} that can be solved very efficiently. Our idea is to replace the constraints that are difficult to satisfy, namely, $x(t) \in \mathcal{X}^{free}$ and $u(t) \in \mathcal{U}$, with a constraint on the time $T$. Intuitively, the constraints on maximum velocity, acceleration, jerk, etc. due to $\mathcal{X}^{obs}$ and $\mathcal{U}$ induce a lower bound on the minimum achievable time in \eqref{eq: problem1}. For example, if the systems's maximum velocity is bounded by $v_{max}$, it cannot reach the goal region faster than $\bar{T}_v:=\frac{d(p_0,\mathcal{P}^{goal})}{v_{max}}$. We describe a procedure for computing a lower bound $\bar{T}$ on the minimum achievable time that takes acceleration and higher-order constraints into account in \TODO{Appendix~\ref{??}}. Hence, to find a heuristic, we replace the state and input constraints, $x(t) \in \mathcal{X}^{free}$ and $u(t) \in \mathcal{U}$, with a lower bound $\bar{T}$ on the minimum time and consider the following Linear Quadratic Minimum-Time Problem~\cite{LQMT}:
\begin{equation}
\label{eq:LQMT}
\begin{aligned}
\min_{D,T} \;& J(D) + \rho T\\
\text{s.t.}\;&\dot{x}(t) = Ax(t)+Bu(t), \quad \forall  t \in [0, T]\\
&x(0) = x_0, \quad x(T) \in \mathcal{X}^{goal}\\
& T \geq \bar{T}
\end{aligned}
\end{equation}
where $A$ and $B$ are defined in \eqref{eq:sys}. Since this is a phyiscally meaningful optimization problem, Bellman's principle of optimality~\cite{bellman2015applied} guarantees that the optimal cost (i.e., the obtained heuristic) will be consistent. The optimal solution to \eqref{eq:LQMT} can be obtained from a minor modification of \cite[Thm.2.1]{LQMT}.

\begin{proposition}
Let $x_f := \argmin_{x \in X^{goal}} \|x_0-x\|$, $\delta_T:= x_f - e^{AT}x_0$, and $G_T:= \int_0^T e^{At} BB^Te^{A^Tt} dt$. Then, the optimal time $T^*$ in \eqref{eq:LQMT} is either $\bar{T}$ or satisfies:
\begin{equation}
-\frac{d}{dT} \crl{\delta_T^T G_T^{-1} \delta_T} = 2x_f^TA^TG_T^{-1}\delta_T + \delta_T^TG_T^{-1}BB^TG_T^{-1}\delta_T = \rho,
\end{equation}
the optimal cost is $\delta_{T^*}^T G_{T^*}^{-1} \delta_{T^*}+\rho T^*$, while the optimal control is:
\[
u^*(t) := B^Te^{A^T(T^*-t)}G_{T^*}^{-1}d_{T^*}
\]
\end{proposition}

Below, we give examples of these expressions for several practical cases.
\subsection{Velocity Control}
\TODO{TODO}
\subsection{Acceleration Control}
\TODO{TODO}
\subsection{Jerk Control}
\TODO{TODO}




\section{Minimum-Time Bounds due to Control Constraints} 
Similarly, if the robot's maximum acceleration is bounded by $a_{max}$, it cannot reach the goal faster than:
\begin{equation}
\begin{aligned}
\min_{T,u(t)} \;& T\\
\text{s.t.}\;& a(t) = u(t), \quad \|u(t)\| \leq a_{max}, \quad \forall  t \in [0, T]\\
& p(0) = p_0, \quad v(0) = v_0\\
& p(T) \in \mathcal{P}^{goal}, \quad v(T) = 0
\end{aligned}
\end{equation}
The above problem is a minimum-time optimal control problem with input constraints, which is difficult to solve directly in 3-D~\cite{mintime_acc_constraint} but can be solved along the individual axes~\cite[Ch.5]{lewisBook}, \cite[Ch.4]{liberzonBook} to obtain times $T_a^1,T_a^2,T_a^3$ (Bang-bang Control of Systems Obeying Newton's Laws) as follows:
\begin{align*}
T_a^1 &:= \frac{1}{a_{max}}\prl{v_i^x + 2 \sqrt{ |p_g^x-p_i^x|a_{max} +(v_i^x)^2 -\frac{(v_i^x)^2a_{max}}{2} }}\\
T_a^2 &:= v_i^y + 2 \sqrt{ |p_g^y-p_i^y| + \frac{(v_i^y)^2}{2} } \quad (\text{ for } a_{max} = 1)\\
T_a^3 &:= v_i^z + 2 \sqrt{ |p_g^z-p_i^z| + \frac{(v_i^z)^2}{2} } \quad (\text{ for } a_{max} = 1)
\end{align*}
This procedure can be continued for the constraints on the higher-order derivatives but the problems become more complicated to solve and the computed times would be less likely to dominate the previous ones. 


%Hence to find a heuristic, we aim to solve the following linear quadratic minimum-time (LQMT) problem~\cite{LQMT}:
%\begin{equation}
%\begin{aligned}
%\min_{B,T} \;& J(B) + \omega T\\
%\text{s.t.}\;&x(0) = x_0, \quad x(T) \in \mathcal{X}^{goal}\\
%& T \geq \max\{T_v,T_a^1,T_a^2,T_a^3\}
%\end{aligned}
%\end{equation}
%in which the state and input constraints, $x(t) \in \mathcal{X}^{free}$ and $u(t) \in \mathcal{U}$, have been replaced with a lower bound on the time. For fixed $T$, and without state and input constraints, the LQMT problem can be readiliy solved~\cite{LQMT} and reduces to:
%\begin{equation}
%\begin{aligned}
%\min_T \; & d_T^TG_T^{-1}d_T + \omega T\\
%\text{s.t.}\;&T \geq \max\{T_v,T_a^1,T_a^2,T_a^3\}
%\end{aligned}
%\end{equation}
%where $d_T:= x_g - e^{AT}x_0$, $G_T := \int_0^T e^{At} B B^T e^{A^Tt} dt$, and
%\begin{equation}
%A = \begin{bmatrix}
%    0 & I & 0 & \cdots &0\\
%    0 & 0 & I & \cdots &0\\
%    \vdots& &\ddots &\ddots&\vdots\\
%    0& \cdots & \cdots & 0 & I\\
%    0& \cdots & \cdots & 0 & 0\\
%    \end{bmatrix} \qquad B = \begin{bmatrix} 0 \\ 0\\\vdots\\0\\I\end{bmatrix}
%\end{equation}
%Hence, the proposed heuristic is: $h(x_0) := d_{T^*}^TG_{T^*}^{-1}d_{T^*} + \omega {T^*}$, where $T^* := \max\{T_v,T_a^1,T_a^2,T_a^3\}$. The explicit heuristic equations for velocity and acceleration control are:
%\begin{align*}
%J_v &= \frac{\|p_g-p_i\|^2}{T^*} +\omega T^*\\
%J_a &=\frac{6\|(p_g-p_i)-T^*v_i\|^2 + 6\|p_g-p_i\|^2 - 2(T^*)^2\|v_i\|^2}{T^*} +\omega T^*\\
%J_j &= \TODO{todo}
%\end{align*}


==> tex/old/LQMT.tex <==
\section{Linear Quadratic Minimum-Time Problem}
\label{sec:lqmt}
In this section, we consider a relaxation of the original problem in Eq.~\eqref{eq: problem1} that can be solved very efficiently and will be used to design motion primitives and a consistent heuristic\footnote{A heuristic function $h$ is \textit{admissible} if it underestimates the optimal cost-to-go from $x_0$, i.e., $0 \leq h(x_0) \leq C^*\prl{x_0,\mathcal{X}^{goal}}, \forall x_0 \in \mathcal{X}$. A heuristic function $h$ is \textit{consistent} if it satisfies the triangle inequality, i.e., $h(x_0) \leq C^*\prl{x_0,\{x_1\}} + h(x_1), \forall x_0,x_1 \in \mathcal{X}$.} for a graph-search solution to Problem~\ref{prob: 1}. Our idea is to replace the constraints that are difficult to satisfy, namely, $x(t) \in \mathcal{X}^{free}$ and $u(t) \in \mathcal{U}$, with a constraint on the time $T$. Intuitively, the constraints on maximum velocity, acceleration, jerk, etc. due to $\mathcal{X}^{obs}$ and $\mathcal{U}$ induce a lower bound $\bar{T}$ on the minimum achievable time in Eq.~\eqref{eq: problem1}. For example, if the systems's maximum velocity is bounded by $v_{max}$, it cannot reach the goal region faster than $\bar{T}_v:=\frac{d}{v_{max}}$ where $d$ is the shortest distance from current position towards the goal.
% More details on how to choose an appropriate lower bound $\bar{T}$ on the minimum achievable time are be provided in \TODO{Appendix~\ref{??}}. 
Hence, we relax Problem~\ref{prob: 1} by replacing the state and input constraints, $x(t) \in \mathcal{X}^{free}$ and $u(t) \in \mathcal{U}$, with a constraint $T \geq \bar{T}$ and consider the following Linear Quadratic Minimum-Time Problem~\cite{LQMT}:
\begin{equation}
\label{eq:LQMT}
\begin{aligned}
\min_{D,T} \;& J(D) + \rho T\\
\text{s.t.}\;&\dot{x}(t) = Ax(t)+Bu(t), \quad \forall  t \in [0, T]\\
&x(0) = x_0, \quad x(T) \in \mathcal{X}^{goal}\\
& T \geq \bar{T}
\end{aligned}
\end{equation}
where $A$ and $B$ are defined in Eq.~\eqref{eq:sys}. The optimal solution to Eq.~\eqref{eq:LQMT} can be obtained from a minor modification of \cite[Thm.2.1]{LQMT}.

\begin{proposition}
\label{prop:LQMT}
Let $x_f\in  \mathcal{X}^{goal}$, $\delta_T:= x_f - e^{AT}x_0$, and $G_T:= \int_0^T e^{At} BB^\T e^{A^\T t} dt$. Then, the optimal time $T$ in \eqref{eq:LQMT} is either the lower bound $\bar{T}$ or the solution of following equation:
\begin{equation}
\scaleMathLine[0.9]{-\frac{d}{dT} \crl{\delta_T^\T G_T^{-1} \delta_T} = 2x_f^\T A^{\T}G_T^{-1}\delta_T + \delta_T^\T G_T^{-1}BB^\T G_T^{-1}\delta_T = \rho}
\end{equation}
The optimal control is:
\begin{equation}
u^*(t) := B^\T e^{A^\T(T-t)}G_{T}^{-1}\delta_{T}
\end{equation}
While the optimal cost is:
\begin{equation}\label{eq:optimal_cost}
C^*(x_0,\{x_f\})=\delta_T^\T G_T^{-1} \delta_T+\rho T
\end{equation}
The explicit form of the polynomial coefficients $D \in \mathbb{R}^{3 \times (2n)}$ is:
\begin{align*}
d_{0:(n-1)} = x_0, \qquad d_{n:(2n-1)} = \delta_T^\T G_T^{-\T}e^{AT}P^\T
\end{align*}
where $P \in \mathbb{R}^{(3n) \times (3n)}$ with $P_{ij} = \begin{cases} (-1)^j, & i=j \\ 0, & i\neq j \end{cases}$
\end{proposition}
Below, we give examples of these expressions for several practical cases with a fixed value of $T$.

\subsection{Velocity Control}
Let $n=1$ so that $\mathcal{X} \subset \mathbb{R}^3$ is position space and $\mathcal{U}$ is velocity space. Then, the optimal solution to Eq.~\eqref{eq:LQMT} according to Proposition~\ref{prop:LQMT} is:
\begin{align*}
d_1 &= \frac{1}{T}\prl{x_f-x_0}\\
x^*(t) &= d_1t + x_0\\
u^*(t) &= d_1\\
C^* &= \frac{1}{T} \|x_f-x_0\|^2 + \rho T
\end{align*}
\subsection{Acceleration Control}
Let $n=2$ so that $\mathcal{X} \subset \mathbb{R}^6$ is position-velocity space and $\mathcal{U}$ is acceleration space. Then, the optimal solution to \eqref{eq:LQMT} according to Proposition~\ref{prop:LQMT} is:
\begin{align}
\begin{pmatrix}
d_2\\d_3
\end{pmatrix} &= \begin{bmatrix}
\frac{6}{T^2} & -\frac{2}{T}\\
-\frac{12}{T^3} & \frac{6}{T^2}
\end{bmatrix}\begin{bmatrix}
p_f-p_0-v_0T\\
v_f-v_0
\end{bmatrix}\nonumber\\
x^*(t) &= \begin{bmatrix}
  \frac{d_3}{6}t^3+\frac{d_2}{2}t^2 + v_0 t + x_0\\
  \frac{d_3}{2}t^2+d_2t + v_0
\end{bmatrix}\label{eq: acc_s}\\
u^*(t) &= d_3t+d_2\label{eq: acc_c}\\
C^* &= \frac{12\|p_f - p_0\|^2}{T^3} - \frac{12(v_0+v_f)\cdot(p_f-p_0)}{T^2} + \nonumber\\
&\frac{4(\|v_0\|^2+v_0\cdot v_1+\|v_1\|^2)}{T}  + \rho T
\end{align}
\subsection{Jerk Control}
Let $n=3$ so that $\mathcal{X} \subset \mathbb{R}^9$ is position-velocity-acceleration space and $\mathcal{U}$ is jerk space. Then, the optimal solution to \eqref{eq:LQMT} according to Proposition~\ref{prop:LQMT} is:
\begin{align}
&\scaleMathLine{\begin{pmatrix}
d_3\\d_4\\ d_5
\end{pmatrix} =  \begin{bmatrix}
\frac{60}{T^3} & -\frac{24}{T^2} & \frac{3}{T}\\
-\frac{360}{T^4} & \frac{168}{T^3} & -\frac{24}{T^2}\\
\frac{720}{T^5} & -\frac{360}{T^4} & \frac{60}{T^3}
\end{bmatrix}\begin{bmatrix}
p_f-p_0-v_0T-\frac{1}{2}a_0T^2\\
v_f-v_0-a_0T\\
a_f-a_0
\end{bmatrix}}\nonumber\\ 
&x^*(t) = \begin{bmatrix}
  \frac{d_5}{120}t^5+\frac{d_4}{24}t^4+\frac{d_3}{6}t^3+\frac{a_0}{2}t^2 + v_0 t + x_0\\
  \frac{d_5}{24}t^4+\frac{d_4}{6}t^3+\frac{d_3}{2}t^2+a_0t+v_0\\
  \frac{d_5}{6}t^3+\frac{d_4}{2}t^2+d_3t+a_0
\end{bmatrix}\label{eq: jrk_s}\\
&u^*(t) = \frac{d_5}{2}t^2+d_4t+d_3\\
&C^* = \TODO{TODO}
\end{align}



% We describe a procedure for computing a lower bound $\bar{T}$ on the minimum achievable time that takes acceleration and higher-order constraints into account in \TODO{Appendix~\ref{??}}. Hence, to find a heuristic, we replace the state and input constraints, $x(t) \in \mathcal{X}^{free}$ and $u(t) \in \mathcal{U}$, with a lower bound $\bar{T}$ on the minimum time and consider the following Linear Quadratic Minimum-Time Problem~\cite{LQMT}. Since this is a phyiscally meaningful optimization problem, Bellman's principle of optimality~\cite{bellman2015applied} guarantees that the optimal cost (i.e., the obtained heuristic) will be consistent.




%If the constraints $x(t) \in \mathcal{X}^{free}$ and $u(t)\in{\mathcal{U}}$ in Problem \eqref{eq: problem1} are removed, we obtain the classical Linear Quadratic Minimum-Time Problem~\cite{LQMT}, which can be solved via Pontryagin's minimum principle~\cite{lewisBook}. In detail, consider the linear time-invariant system $\dot{x} = Ax+Bu$ with 
%\begin{equation}
%A = \begin{bmatrix}
%    0 & I & 0 & \cdots &0\\
%    0 & 0 & I & \cdots &0\\
%    \vdots& &\ddots &\ddots&\vdots\\
%    0& \cdots & \cdots & 0 & I\\
%    0& \cdots & \cdots & 0 & 0\\
%    \end{bmatrix} \qquad B = \begin{bmatrix} 0 \\ 0\\\vdots\\0\\I\end{bmatrix}
%\end{equation}





==> tex/old/TrajectoryPlanning_old.tex <==
\section{Deterministic Optimal Trajectory Planning}
\label{sec: planning}
\subsection{Problem Revisit}
A trajectory $x(t)$ can be divided into $N$ short trajectory segments $x_k(\tilde{t})$. Without loss of generality, we look into the problem in which each short trajectory segment has the same time period as $\tau$ such that $\tilde{t}\in[0, \tau]$. As a result, the total time of $x(t)$ is equation to the multiplication of number of short segments and their execution time:
\begin{equation}
T = \sum_{i=0}^{N-1} \tau = N\tau
\end{equation}


Considering the state space $\mathcal{X}^{free}$ is spanned as a graph $\mathcal{G}(S, E)$ with our predefined motion primitives. Let $x_k(\tilde{t})$ be the short trajectory that connects two nearby states $s_k, s_{k+1}$ in $S$, from the previous discussion we know that its cost $C(x_k)$ has the lower bound which is defined by our discretized primitive that connects the same states (eq.~\eqref{eq: Cl}).
\begin{equation}\label{eq: Cl}
C(x_k,u_k) \geq  (\|u_{k}\|^2 + \rho) \tau
\end{equation}

Thus, we consider the following constrained version (the control input is constrained to be piecewise-constant) of the original problem in eq.~\eqref{eq: problem1}.
%Thus, the original problem in eq.~\eqref{eq: problem1} is equivalent to the following simpler problem

\begin{problem}\label{prob: 2}
Given an initial state $x_0 \in \mathcal{X}^{free}$ and a goal region $\mathcal{X}^{goal} \subset \mathcal{X}^{free}$ and a finite set of motion primitives $\mathcal{U}_M$ with duration $\tau$, choose a sequence of motion primitives $u_{0:N-1}$ such that:
\begin{equation}
\label{eq: problem3}
\begin{aligned}
\min_{N, u_{0:N-1}} \;& \prl{\sum_{k=0}^{N-1}  \|u_k\|^2 + \rho N}\tau\\
\text{s.t.}\;&u_{k} \in \mathcal{U}_M, \quad \forall k \in [0,\ldots,N-1]\\
&x_{k}(\tilde{t}) = f(s_k, u_k) \subset \mathcal{X}^{free}, \quad \forall  \tilde{t} \in [0, \tau]\\
&s_{k+1} = x_k(\tau)\\
&s_0 = x_0, \quad s_{N} \in \mathcal{X}^{goal}
\end{aligned}
\end{equation}
\end{problem}

% solvable within the framework of graph search. We present the solution in this section with properly designed heuristic function and collision checking methods.
The re-formulation of original Problem~\ref{prob: 1} as Eq.~\eqref{eq: problem3} is an instance of a deterministic shortest path problem~\cite{OptimalControlBook} with discrete control and state spaces. Such problems can be solved via search-based~\cite{hart1968formal,ara_star}  or sampling-based~\cite{Lavalle98rapidly-exploringrandom,rrt-star,arslan2013use} motion planning algorithms. Since only the former guarantee finite-time (sub-)optimality, we use an A* method and focus on the design of an accurate, consistent heuristic and efficient, guaranteed collision checking methods. A consistent heuristic function allows reaching the goal region faster without loss of optimality. Also, since the collision checking is always the most expensive part in motion planning, we provide two efficient approaches that guarantee trajectory safety.

\subsection{Graph Construction}
Conventionally, the graph is defined as $\mathcal{G}(S, E)$ where $S$ stands for the set of feasible nodes $S := \{s_q\in \mathcal{X}^{free}\;|\;q=0,1,\ldots\}$ and $E$ stands for the set of edges that connect the graph $E := \{e_q^r(t) \subset \mathcal{X}^{free} \;|\; s_q = e_q^r(0), s_r = e_q^r(\tau) \in S\}$. We define the edge between two nodes $s_q, s_r$ as the motion primitive defined in previous section. Define the corresponding discretized state of a given initial state $x_0$ as $s_0$, the graph $\mathcal{G}$ is constructed using $s_0$ and user defined discretized control inputs $\mathcal{U}_M$. The resolution for state discretization is mentioned before in Section.~\ref{sec:dis}.

We use Algorithm~\ref{alg: succ} to explore the free state space $\mathcal{X}^{free}$ and build the connected graph: in line 4, the primitive is calculated using the fully defined state $s_q$ and a control input $u_m$ given the constant time $\tau$; line 5 checks the feasibility of the primitive, this step will be further discussed in Section.~\ref{sec: col}; in line 6, we evaluate the end state of a valid primitive and add it to the set of successors of the current node; in the meanwhile, we estimate the edge cost as defined in Eq.~\eqref{eq: C} from the corresponding primitive. After checking through all the primitives in the finite control input set, we add the nodes in successor set $\mathcal{S}(s_q)$ to the graph, and we continue expanding until reaching the goal region.
\begin{algorithm}[h!]
\caption{Given the current state $s_q$, and a set of control input $\mathcal{U}_M$ with time $\tau$, find its successors $\mathcal{S}(s_q)$. \label{alg: succ}}
\begin{algorithmic} [1]
\Function{GetSuccessors}{$s_q,\mathcal{U}_M, \tau$}
\State $\mathcal{S}(s_q) \gets \emptyset$
\ForAll{$u_m \in \mathcal{U}_M$}
\State $e_q^m \gets f(s_q, u_m)$
\If {$e_q^m \subset \mathcal{X}^{free}$}
\State $s_m \gets e_q^m(\tau)$
\State $\mathcal{S}(s_q) \gets s_m, C(e_q^m)$
\EndIf
\EndFor
\State\Return {$\mathcal{S}(s_q)$}
\EndFunction
\end{algorithmic}
\end{algorithm}


\subsection{Heuristic Function}\label{sec:heur}
We define a goal node $s_g = [p_g^\T, v_g^\T, a_g^\T, ...]^\T$ centered at the goal region for calculating the heuristic for nodes in $\mathcal{G}$. According to Eq.~\eqref{eq: problem0}, the the cost from current state $s_q$ to goal $s_g$ is
\begin{equation}
C(s_q, s_g) = \int_0^{\tau_g} \| p^{(n)}_{D_{q, g}}(t)\|^2 dt + \rho {\tau_g}
\end{equation}

Let $\tau_g$ be the time to reach the goal regardless of obstacles, we are looking for heuristic functions that are both \textit{admissible} and \text{consistent} to ensure the algorithm optimality. In this section, we provide two choices of heuristic functions that satisfy the requirement.

\subsubsection{Maximum Speed Heuristic}
When the maximum allowed speed $v_{max}$ is set for our system, we can defined the heuristic function as
\begin{equation}\label{eq: h1}
h(s_q) = \rho\tau^* = \rho \frac{\|p_g - p_q\|_\infty}{v_{max}}
\end{equation}
Here $\tau^*$ indicates the smallest time that a robot can traverse to the goal position. The infinity norm assume the speed limits are forced for each axis independently. It is easy to see that Eq.~\eqref{eq: h1} is \textit{consistent} due to triangle inequality in distance. It is also straight-forward to verify \textit{admissible} as
\begin{align*}
C(s_q, s_g) \geq \rho \tau_g \geq \rho \tau^*=h(s_q)
\end{align*}

\subsubsection{Minimum Cost Heuristic}
The \textit{Max Speed Heuristic} does not work well when the maximum speed is set to be very large. As $v_{max}\rightarrow \infty$, $h(s_q)\rightarrow 0$ which turns the algorithm into Dijkstra. Removing the constraints on system's dynamics allow us to solve for the optimal trajectory from current state $s_q$ to the goal state $s_g$, this trajectory is the minimum cost trajectory such that its cost can be used as another choice of heuristic function. This minimum cost is discussed in Sec.~\ref{sec:lqmt} and it has the form of Eq.~\eqref{eq:optimal_cost} as
\begin{equation}\label{eq: hhh2}
h(s_q) = C^*(s_q,\{s_g\})=\delta_T^\T G_T^{-1} \delta_T+\rho T
\end{equation}
Here the optimal time $T$ can be solved as
\begin{equation}\label{eq:time_opt}
T = \argmin_{\tau_g}  \int_{0}^{\tau_g} \left\|u(t)\right\|^2 dt + \rho \tau_g
\end{equation}

For \textit{Kinematic Model},  let $s_q = [p_q^\T, v_q^\T]^\T, s_g = [p_g^\T, v_g^\T]^\T$, Eq.~\eqref{eq: hhh2} turns out to be the root of a $4$-th order polynomial by taking the derivative of the cost function with respect to $T$ as
\begin{equation}
0 = c_4 T^4 + c_3 T^3 + c_2 T^2+c_1T+c_0
\end{equation}
where
\begin{align*}
c_0 &= -3\|p_g-p_q\|^2\\
c_1 &= 24(v_q+v_g)\cdot(p_g - p_q)\\
c_2 &= -4(\|v_q\|^2+v_q\cdot v_g + \|v_g\|^2)\\
c_3 &= 0, \quad c_4 = \rho
\end{align*}

This heuristic function is also valid as: first, it underestimates the actual cost since we remove the constraints on dynamics and obstacles when calculating; second, $\tau^*$ gives the optimal control $u^*(t)$ to make sure the consistency.


\subsection{Collision Checking}\label{sec: col}
For a given edge $e(t) = [p(t)^\T, v(t)^\T, a^\T, ...]^\T$ in $\mathcal{G}$, we need to check if $e\subset \mathcal{X}^{free}$. As we define the state space in $\mathbb{R}^{3n}$, we separate the collision checking in a geometric space in $\mathcal{M}^{free} \subset \mathbb{R}^3$ and in a kinodynamic space $\mathcal{D}^{free} \subset \mathbb{R}^{3(n-1)}$ where $\mathcal{X}^{free} = \mathcal{M}^{free}\cup\mathcal{D}^{free}$. $e$ is valid only if its geometric shape $p$ is inside the free space and derivatives $(v, a, ...)$ are bounded by kinodynamic constraints as
\begin{equation}
e = [p, v, a, ...]\subset \mathcal{X}^{free} \iff \left. \begin{array}{l}
         p\subset \mathcal{M}^{free}\\
         (v,a, ...)\subset \mathcal{D}^{free}\end{array}\right.
\end{equation}

As $(v, a, ...)$ are defined as polynomials, we can calculate their extrema within the time period $[0, \tau]$ and compare them with maximum bounds on velocity, acceleration, etc. For $n \leq 3$, the order of those polynomials are smaller than $5$, which means we can easily solve the extrema in closed form. Denote max magnitude of velocity, acceleration as $v_{max}, a_{max}$, we have

\begin{equation}
(v,a, ...)\subset \mathcal{D}^{free}   \Leftrightarrow\left. \begin{array}{ll}
         \|v\|_{\infty} \leq v_{max}, & \forall t\in[0, \tau]\\
         \|a\|_{\infty} \leq a_{max}, & \forall t\in[0, \tau]\\
         \vdots&\end{array}
         \right.
\end{equation}

The harder part is checking collision in $\mathcal{M}^{free}$. Here we discuss efficient checking process in \textit{Occupancy Grid Map}. Other possible approaches like \textit{Polyhedral Map} are also considered to be efficient, but they're usually hard to get from real-world sensor data(~\cite{deits2015computing},~\cite{liu2016high}) and the quality of the map decomposition is very important to the completeness of the trajectory planning. In this paper, we mainly discuss the simple but effective collision checking using the \textit{Occupancy Grid Map} which is one of the most popular kinds of map researchers utilize for navigation. It discretizes the environment in $\mathbb{R}^2$ or $\mathbb{R}^3$ into a grid w.r.t certain map resolution $R$. For example, let $p$ be a 2-D position in $\mathbb{R}^2$, $c(p) = c_{(n_x, n_y)} = [n_x, n_y]$ gives the discretized coordinates of $p$ in the map. A grid cell $c(p)$ is represented as $free, occupied, unknown$ regarding the value $V(c)$ on this cell. In this case, $\mathcal{M}^{free} = \{c_{(n_x, n_y)}\;|\;V(c) = free, n_x = 0,\ldots,N_x, n_y = 0,\ldots,N_y \}$, where $N_x, N_y$ stand for the dimension of the map in $x, y$ axis.

Let $\mathcal{P} := \{p_0, p_1,\ldots,p_D\}$ be the set of a sequence of position that a robot traverses along the trajectory $p(t)$. To ensure collision-free, we need to ensure that all $p_d \in \mathcal{P}$ are $free$ (Eq.~\ref{eq: free}).
\begin{equation}\label{eq: free}
p(t)\subset\mathcal{M}^{free}\iff \forall p_d \in \mathcal{P},\; V(c(p_d)) = free
\end{equation}
We sample  $\mathcal{P}$ from a given trajectory $p(t)$ with duration $T$ as
\begin{align*}
p_d =\;& p(t_d)\\
 t_d =\;& \frac{d}{D}T, \;\forall d = 0, 1,\ldots, D
\end{align*}
The number $D$ defines how many samples we want to check on a trajectory. Denote $v_{max}$ as the maximum speed in one axis, we conclude that $D$ should satisfy following condition to guarantee safety:
\begin{equation}
 D \geq \frac{T}{R}v_{max}
\end{equation}
It makes sure that the maximum distance between two consecutive samples will not exceed the map resolution. It is an optimistic approximation as we ignore several cells that cloud be partially traversed by the trajectory, but it prevents the trajectory penetrating or hitting obstacles.





